The ribbon category framework for topological quantum computing

This expository article supplies the mathematical background underpinning the braid representation calculator introduced in arXiv:2212.00831; those representations describe the sets of logic gates available to a topological quantum computer for processing encoded qubits. Assuming little background in category theory, we first recall the notion of a ribbon fusion category (RFC), collecting most of the necessary definitions. Then we discuss how certain RFCs arise from the representation theory of quantum groups. We explore the braiding in these categories in detail, since it is essential for the quantum computing application.

==> source/rfc_framework/diagram_calc.tex <==
A remarkable feature of a ribbon category is that its morphisms may be understood in terms of certain tangle diagrams. Explaining this correspondence requires a presentation of the category $\mathcal{RIBBON}$ of oriented framed tangle diagrams in terms of generators and relations \cite[Chapter~XII]{Kassel}.
\begin{thm}{\cite[Lemmas~5.2,5.3]{reshetikhin_turaev_1990}}\label{ribbon category generators and relations}
	Every oriented framed tangle diagram is the composition of tensor products of the eight tangles $X_+$, $X_-$, $\overset{\rightarrow}{\cap}$, $\overset{\leftarrow}{\cap}$, $\underset{\rightarrow}{\cup}$, $\underset{\leftarrow}{\cup}$, $\downarrow$, and $\uparrow$, and the composition is completely determined by the monoidal structure and the relations in \Cref{ribbon category relations}.
\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.75]{chapters/prelude/rfc_framework/ribbon_cat_rels.png}
	\caption{Relations between generators in $\mathcal{RIBBON}$.}
	\label{ribbon category relations}
\end{figure}
\end{thm}

With this purely algebraic presentation of $\mathcal{RIBBON}$ in hand, we can state the correspondence between tangle diagrams and morphisms in any ribbon category precisely as the following theorem.

\begin{thm}{\cite[Theorem~2.5]{rt_3_manifolds}}\label{univ prop ribbon category}
	Let $\mathcal{C}$ be a ribbon category and let $V$ be an object of $\mathcal{C}$. Then there exists a unique covariant tensor functor $\mathcal{F}_V: \mathcal{RIBBON} \to \mathcal{C}$ preserving the braiding, the left duality, and the twist, such that $\mathcal{F}_V(+) = V$ and $\mathcal{F}_V(-) = V^*$, and
	\begin{align*}
		\mathcal{F}_V(\downarrow) = \id_V, \quad \mathcal{F}_V(\uparrow) = \id_{V^*}, \quad \mathcal{F}_V(X_+) = c_{V,V}, \quad \mathcal{F}_V(X_-) = \inv{c_{V,V}} \\
		\mathcal{F}_V(\overset{\rightarrow}{\cap}) = d_V, \quad \mathcal{F}_V(\overset{\leftarrow}{\cap}) = d_V', \quad \mathcal{F}_V(\underset{\rightarrow}{\cup}) = b_V, \quad \mathcal{F}_V(\underset{\leftarrow}{\cup}) = b_V'.
	\end{align*}
\end{thm}
\begin{proof}
	For details, see e.g., Chapters~XII-XIV in \cite{Kassel}.	
\end{proof}

When considering RFCs, semisimplicity allows for \textit{fusion}, that is, morphisms of the form $V \otimes W \to X$. We account for these in the diagrammatical framework by allowing trivalent vertices:
\begin{equation*}
\begin{tikzpicture}[scale=0.5]
	\node[scale=1] at (6.5, -1.75) {$\in \Hom(V \otimes W, X)$};
	\fusiontree{2}{{0,0}}
	\outerlab{{V,W}}{X}
\end{tikzpicture}
\end{equation*}
Thus morphisms in RFCs are modeled by oriented framed trivalent graphs.
